From Examples to Rules: Neural Guided Rule Synthesis for Information Extraction

While deep learning approaches to information extraction have had many successes, they can be difficult to augment or maintain as needs shift. Rule-based methods, on the other hand, can be more easily modified. However, crafting rules requires expertise in linguistics and the domain of interest, making it infeasible for most users. Here we attempt to combine the advantages of these two directions while mitigating their drawbacks. We adapt recent advances from the adjacent field of program synthesis to information extraction, synthesizing rules from provided examples. We use a transformer-based architecture to guide an enumerative search, and show that this reduces the number of steps that need to be explored before a rule is found. Further, we show that without training the synthesis algorithm on the specific domain, our synthesized rules achieve state-of-the-art performance on the 1-shot scenario of a task that focuses on few-shot learning for relation classification, and competitive performance in the 5-shot scenario.

==> figures/data-generation-example.tex <==
\begin{tikzpicture}
  % \draw[help lines] (0,0) grid (12,10);
  \def\ya{6}
  \def\yb{4}
  \def\yc{2}

  % first sentence
  \node (w1) at (1.08, \ya) {the};
  \node (w2) at (2, \ya) {rain};
  \node (w3) at (3, \ya) {caused};
  \node (w4) at (4, \ya) {flood};

  \node (l1) at (1.08, \ya-.49) {\textit{the}};
  \node (l2) at (2, \ya-.5) {\textit{rain}};
  \node (l3) at (3, \ya-.55) {\textit{cause}};
  \node (l4) at (4, \ya-.54) {\textit{flood}};

  \node[draw, rounded rectangle] (t1) at (1.08, \ya-1) {\tiny DET};
  \node[draw, rounded rectangle] (t2) at (2, \ya-1) {\tiny NOUN};
  \node[draw, rounded rectangle] (t3) at (3, \ya-1) {\tiny VERB};
  \node[draw, rounded rectangle] (t4) at (4, \ya-1) {\tiny NOUN};
  
  \node[draw, rounded rectangle, rotate=270, thick] at (0.2, \ya-.5) {\small $random(s)$};

  % second sentence
  \node (w1) at (1.08, \yb-.02) {heavy};
  \node (w2) at (2, \yb) {rain};
  \node (w3) at (3, \yb) {caused};
  \node (w4) at (4, \yb) {flood};

  \node (l1) at (1.08, \yb-.49) {\textit{heavy}};
  \node (l2) at (2, \yb-.5) {\textit{rain}};
  \node (l3) at (3, \yb-.545) {\textit{cause}};
  \node (l4) at (4, \yb-.54) {\textit{flood}};
  
  \node[draw, rounded rectangle] (t1) at (1.08, \yb-1) {\tiny ADJ};
  \node[draw, rounded rectangle] (t2) at (2, \yb-1) {\tiny NOUN};
  \node[draw, rounded rectangle] (t3) at (3, \yb-1) {\tiny VERB};
  \node[draw, rounded rectangle] (t4) at (4, \yb-1) {\tiny NOUN};
  
  \node[draw, rounded rectangle, rotate=270, minimum width=1cm, thick] at (0.2, \yb-.5) {\small or};

  % third sentence
  \node (w2) at (1.5, \yc) {rain};
  \node (w3) at (2.5, \yc-.05) {causes};
  \node (w4) at (3.5, \yc) {flood};

  \node (l2) at (1.5, \yc-.5) {\textit{rain}};
  \node (l3) at (2.5, \yc-.545) {\textit{cause}};
  \node (l4) at (3.5, \yc-.54) {\textit{flood}};
  
  \node[draw, rounded rectangle] (t2) at (1.5, \yc-1) {\tiny NOUN};
  \node[draw, rounded rectangle] (t3) at (2.5, \yc-1) {\tiny VERB};
  \node[draw, rounded rectangle] (t4) at (3.5, \yc-1) {\tiny NOUN};
  
  \node[draw, rounded rectangle, rotate=270, minimum width=1cm, thick] at (.2, \yc-.5) {\small ?};

  % rules
  \node at (7.8, \ya-.25) {\small``[tag=DET] [lemma=rain]};
  \node at (7.8, \ya-.65) {\small [lemma=cause] [word=flood]''};
  
  \node at (7.8, \yb-.1) {\small ``\textbf{[tag=DET $|$ tag=ADJ]}};
  \node at (7.8, \yb-.5) {\small ``[lemma=rain] [lemma=cause]};
  \node at (7.8, \yb-.9) {\small [word=flood]''};
  
  \node at (7.8, \yc-.1) {\small ``\textbf{[tag=DET $|$ tag=ADJ]?} };
  \node at (7.8, \yc-.5) {\small [lemma=rain] [lemma=cause]};
  \node at (7.8, \yc-.9) {\small [word=flood]''};
  
  \node[draw, circle] at (10.3, \ya) {1};
  \node[draw, circle] at (10.3, \yb) {2};
  \node[draw, circle] at (10.3, \yc) {3};
 

  \draw[dashed] (5.2, \yc+.5) rectangle (10.8, \yc-1.8);
  \node[dashed] at (8, \yc-1.4) {\small Final Rule};
  %\draw[decorate,decoration={brace,amplitude=10pt,mirror}] (-0.4,\ya) -- (-0.4,\yc-1);
  

  %\draw[thick, ->] (4.6,\ya-.5) to[out=0,in=180] (6,\ya-.5);
  %\draw[thick, ->] (4.6,\ya-.5) -- (4.73, \ya-.5) to[out=0,in=140] (5.8,\yb);
  %\draw[thick, ->] (4.6,\ya-.5) to[out=0,in=140] (5.8,\yc);
 
  %\draw[thick, dashed, ->] (4.6,\yb-.5) to[out=0,in=180] (5.8,\yb-.5);
  %\draw[thick, dashed, ->] (4.6,\yb-.5) to[out=0,in=160] (5.8,\yc-.25);

  %\draw[thick, dotted, ->] (4.3,\yc-.5) to[out=0,in=180] (5.8,\yc-.5);
\end{tikzpicture}


==> figures/data-generation-flowchart.tex <==
\begin{tikzpicture}
  %\draw[help lines] (0,0) grid (12,10);
  \def\y{1}
  
  \node[draw, rounded rectangle] (random) at (2.5, \y) {\tiny random(s)};
  \node[draw, diamond] (coin1) at (3.8, \y) {\tiny ~};

  \node[draw, rounded rectangle] (mod) at (5, \y) {\tiny modifier};
  \node[draw, rounded rectangle] (or) at (5, \y-.8) {\tiny or};
  \node[draw, rounded rectangle] at (5, \y+.6) {\tiny stop};
  \node[draw, rounded rectangle, minimum width=1.1cm, minimum height=.5cm] (stop) at (5, \y+.6) {};

  \node[draw, diamond] (coin2) at (6, \y) {\tiny ~};

  \node[draw, rounded rectangle] (star) at (7, \y+.5) {\tiny *};
  \node[draw, rounded rectangle] (plus) at (7, \y) {\tiny +};
  \node[draw, rounded rectangle] (question) at (7, \y-.5) {\tiny ?};
  
  \draw[-latex] (random) -- (coin1);
  \draw[-latex] ($(random)-(1.1,0)$) -- (random);
  
  \draw[-latex] (coin1) -- (mod);
  \draw[-latex] (coin1) to[out=0,in=180] (stop);
  \draw[-latex] (coin1) to[out=0,in=180] ($(or) - (0.4,0)$) -- (or);

  \draw[-latex] (mod) -- (coin2);
  \draw[-latex] (coin2) -- (plus);
  \draw[-latex] (coin2) to[out=0,in=180] (star);
  \draw[-latex](coin2) to[out=0,in=180] (question);

  \coordinate (exit) at (7.7, \y) {};
  \draw (star) to[out=0,in=180] (exit);
  \draw (plus) -- (exit);
  \draw (question) to[out=0,in=180] (exit);
  \draw (or) -- ($(or) + (2.2,0)$) to[out=0, in=180] (exit);
  
  \draw[-latex] (exit) to[out=0, in=0] ($(exit) + (0,1)$) -- ($(exit) + (-3.6,1)$) to[out=180, in=90] (coin1);

\end{tikzpicture}


==> figures/scoring_example.tex <==
\begin{tikzpicture}
  \def\ya{6}
  \def\yb{4}
  \def\yc{2}
  
  % rules
  \node at (8.2, \ya-.25) {\small``[tag=DET] [lemma=rain]};
  \node at (8.2, \ya-.65) {\small [lemma=cause] [word=flood]''};
\end{tikzpicture}

==> tables/ast_costs.tex <==
\begin{tabular}{ll}
Node Type          & Cost \\ \hline
Hole Matcher        & 2    \\
Hole Constraint     & 3    \\
Hole Query          & 2    \\
String Matcher      & 1    \\
Field Constraint    & 0    \\
Not Constraint      & 10   \\
And Constraint      & 4    \\
Or Constraint       & 4    \\
Token Query         & 0    \\
Concat Query        & 4    \\
Or Query            & 4    \\
Repeat Query        & 15   \\
Match All Matcher    & 0    \\
Match All Query      & 0    \\
Match All Constraint & 0   
\end{tabular}

==> tables/intrinsic.tex <==
{\footnotesize
\begin{tabular}{l|rr|rr}
\multicolumn{1}{c|}{\multirow{2}{*}{Execution}} & \multicolumn{2}{c|}{With Reward}                                                                                                                               & \multicolumn{2}{c}{Without Reward}                                                                                                                           \\
\multicolumn{1}{c|}{}                           & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Static\\ Weight\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Contextual\\ Weight\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Static\\ Weight\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Contextual\\ Weight\end{tabular}} \\ \hline
Timeout                                         & 1k states                                                                   &                                                                                  & 1k states                                                                   & 1k states                                                                       \\
Rules found                                     & 581/1000                                                                    &                                                                                  & 283/1000                                                                    & 864/1000                                                                        \\
Ceiling avg                                     & 12.0                                                                        &                                                                                  & 12.0                                                                        & 12.2                                                                            \\
Ceiling median                                  & 14.0                                                                        &                                                                                  & 14.0                                                                        & 14.0                                                                            \\
Ceiling max                                     & 24                                                                          &                                                                                  & 24                                                                          & 29                                                                              \\
Ceiling min                                     & 9                                                                           &                                                                                  & 9                                                                           & 9                                                                               \\
Steps avg                                       & 95.1                                                                        &                                                                                  & 424.2                                                                       & 21.3                                                                            \\
Steps median                                    & 46.0                                                                        &                                                                                  & 348.0                                                                       & 17.0                                                                            \\
Steps max                                       & 676                                                                         &                                                                                  & 999                                                                         & 734                                                                             \\
Steps min                                       & 13                                                                          &                                                                                  & 87                                                                          & 9                                                                              
\end{tabular}
}

==> tables/intrinsic_tacred.tex <==
{\footnotesize
\begin{tabular}{l|rr|rr}
\multicolumn{1}{c|}{\multirow{2}{*}{Execution}} & \multicolumn{2}{c|}{With Reward} & \multicolumn{2}{c}{Without Reward} \\
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Static\\ Weight\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Contextual\\ Weight\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Static\\ Weight\end{tabular}} &
  \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Contextual\\ Weight\end{tabular}} \\ \hline
Timeout                                         &                 &                & 1k states        & 1k states        \\
Rules found                                     &                 &                & 673/3928         & 1392/3928        \\
Steps avg                                       &                 &                & 323              & 195              \\
Steps median                                    &                 &                & 189              & 58.5             \\
Steps max                                       &                 &                & 972              & 1000             \\
Steps min                                       &                 &                & 18               & 10              
\end{tabular}
}

==> tables/static_scorer_example.tex <==
\begin{tabular}{lllllll}
     & JJ           & JJ                & NNS     & MD  & RB    & VB    \\
s1  & Green        & great             & dragons & can & not   & exist \\
     &              &                   &         &     &       &       \\
     & JJ           & JJ                & NNS     & MD  & VB    &       \\
s2  & Great        & green             & dragons & can & exist &       \\
     &              &                   &         &     &       &       \\
cs   & {[}tag=JJ{]} & {[}word={$\square$}{]} & {$\square$}  &     &       &       \\
nps1 & {[}tag=JJ{]} & {[}word=great{]}  & {$\square$}  &     &       &       \\
nps2 & {[}tag=JJ{]} & {[}word=green{]}  & {$\square$}  &     &       &      
\end{tabular}

==> tables/static_scorer_example2.tex <==
\begin{tabular}{lcccl}
     & JJ                               & JJ                                   & NNS                    & ... \\
s1   & Green                            & great                                & dragons                & ... \\
     &                                  &                                      &                        &     \\
     & JJ                               & JJ                                   & NNS                    & ... \\
s2   & Great                            & green                                & dragons                & ... \\
     & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}   &     \\
cs   & \multicolumn{1}{l}{{[}tag=JJ{]}} & \multicolumn{1}{l}{{[}word=$\square${]}}      & $\square$ &     \\
nps1 & \multicolumn{1}{l}{{[}tag=JJ{]}} & \multicolumn{1}{l}{{[}word=great{]}} & $\square$ &     \\
nps2 & \multicolumn{1}{l}{{[}tag=JJ{]}} & \multicolumn{1}{l}{{[}word=green{]}} & $\square$ &    
\end{tabular}

==> tables/tacred.tex <==
{\footnotesize
\begin{tabular}{llll}
    \toprule
Model                           & P    & R    & F1   \\ \midrule
\multicolumn{4}{c}{Baselines}                        \\ \midrule
Seq2Seq with Transformers       & 53.0 & 19.0 & 28.0 \\ 
Manual patterns \cite{Angeli2015BootstrappedST} & 86.9 & 23.2 & 36.6 \\ % \cite{Angeli2015BootstrappedST}
% No Learning                     & 53.0 & 19.0 & 28.0 \\ 
\midrule
\multicolumn{4}{c}{Supervised Approaches}              \\ \midrule
    \citet{joshi-etal-2020-spanbert} & 70.8 &  70.9 & 70.8 \\
    \citet{zhou2021improved}        & -- & -- & 74.6 \\
    \citet{cohen2020relation}       & 74.6 & 75.2 & 74.8 \\ \midrule
% Logistic Regression (LR)        & 73.5 & 49.9 & 59.4 \\
% LR + Patterns                   & 72.9 & 51.8 & 60.5 \\
% CNN                             & 75.6 & 47.5 & 58.3 \\
% LSTM                            & 65.7 & 59.9 & 62.7 \\
% LSTM + Position-aware attention & 65.7 & 64.5 & 65.1 \\ \midrule
\multicolumn{4}{c}{Our approach}                     \\ \midrule
Static weights                   & 54.9 & 24.6 & 34.0 \\
Static weights with reward       & 56.1 & 24.9 & 34.5 \\
Contextual weights (BERT-Tiny)   & 57.6 & 29.6 & 39.1 \\
Contextual weights (BERT-Mini)   & 57.2 & 32.5 & 41.4 \\
Contextual weights (BERT-Small)  & 57.3 & 32.2 & 41.2 \\
Contextual weights (BERT-Medium) & 55.0 & 31.8 & 40.3 \\
Contextual weights (BERT-Base)   & 55.6 & 32.4 & 41.0 \\
\bottomrule
\end{tabular}
}


==> tex/data-generation.tex <==

% ms: there are no other paragraphs in this section...
%\paragraph{Training data} 
%\label{sssp:training_data}


% We generate data by first running the system with the static weights scorer.
% We extract a random number of random sentences from the UMBC corpus.
% We then select a random span from each sentence to serve as the highlighted portion.\footnote{Some smarter ways to ensure there exists a rule (other than a concatenation of ORs): favoring spans that have something common (a part-of-speech tag, for example), favoring noun phrases (NPs), etc.} 
% We then run our system with the \textit{static weights} approach to generate a rule.
% For diversity,
% between each rule generation we reinitialize the costs of each type of state randomly.
% For example, in one run we might have 
% $cost(\square)=2$,
% $cost(concatenation)=3$
% and $cost(\square ~ \square) 
% = cost(\square) + cost(\square) + cost(concatenation) = 7$, 
% while in the next run we might have $cost(\square)=1$,
% $cost(concatenation)=4$ 
% and $cost(\square ~ \square) = 
% cost(\square) + cost(\square) + cost(concatenation) = 6$. 
% This ensures that we do not generate data that 
% is biased towards a certain type of rules.
Specifically, 
we iteratively generate training rules from the UMBC corpus \citelanguageresource{han2013umbc}. 
% using the algorithm in Figure~\ref{data-generation-flowchart}.
%
% We generate data using odinson and the UMBC corpus.
% First, we index the UMBC corpus using odinson.
% Thereafter we apply the algorithm presented in 
% Figure~\ref{data-generation-flowchart}
% to iteratively generate the rules.
We first randomly select a sentence from this corpus,
and from that sentence we select a random span (of random length).
Then,
for each token in the span,
we randomly choose whether to use the \textit{lemma, word,}
or \textit{part-of-speech (POS) tag} for its representation.
These correspond to the token constraints that can be used in the rules.  
To enable the learning of rules that contain concatenation and/or token constraints, 
we need to perform additional modifications in order 
to expose the contextualized searcher to the other available components of rules.  
To do this,
we iterate over a loop that randomly decides whether
to stop or continue and add a modifier \todo{Becky/George: this sentence is not clear: what is "iterate over a loop"? do you mean stop the whole rule, or just the addition of other components?}
(e.g., inserting an disjunction
or a quantifier such as \texttt{*, +} or \texttt{?}).
Modifiers are added by first randomly
selecting the position at which to intervene 
and then the type of intervention (alternation or quantification).
To add an alternation, 
we substitute the rule element in that position 
with a wildcard and search the corpus for another sentence 
that has different content in that position.
To add quantification,
we randomly decide which quantifier to add,
and then query the corpus to ensure that through the addition we are,
in fact, able to match additional sentences.  
% This process is illustrated in Figure \ref{data-generation-example}.

% \begin{figure}[H]
%   \centering
%   \resizebox{\columnwidth}{!}{
%     \input{figures/data-generation-flowchart}
%   }
%   \caption{
%     The set of steps used to automatically generate the random 
%     rules for the training data.
%     First we randomly select a sentence from UMBC.
%     Afterwards we randomly choose a span to represent 
%     the portion of the sentence that should be extracted by the rule.
%     For each token selected we throw a coin 
%     to decide which representation to use: lemma, word or part-of-speech (POS) tag.
%     Subsequently we iterate over a loop that
%     throws a coin to select the action to take:
%     stop, add a modifier or add an or.
%   }
% \label{data-generation-flowchart}
% \end{figure}

After each rule is finished, we then query the UMBC corpus with it to obtain additional 
sentences (and the span they match) to generate a multi-sentence specification.
% Figure~\ref{data-generation-example} shows 
% an example of a rule generated in three steps.
% The final result of one iteration 
% is a sequence of positive examples
% and the rule that satisfy them.
Note that the rule and example sentences and spans also need to satisfy
the heuristics used to prune the search space. \todo{Becky/George: unclear. what heuristics? point to the correct subsection.}

% \begin{figure}[H]
%   \centering
%   \resizebox{\columnwidth}{!}{
%     \input{figures/data-generation-example}
%   }
%   \caption{
%     An example of a rule generated using our approach.
%     Line one shows the first step: select the random sentence.
%     The randomly selected sentence is used to generate the rule 1.
%     In this example, the whole sentence is marked to be extracted by the rule.
%     In the second row, we show the addition of an alternation.
%     % Adding the or is done by throwing a coin 
%     % to select the position $i$ where the rule will be changed
%     and searching for a sentence that is different at that position (rule 2).
%     Finally, line three adds a quantifier, \texttt{?}, and checks to see
%     % Adding a modifier is done by throwing a coin to select $i$,
%     % adding the the modifier to the rule and checking 
%     if it is able to extract a new sentence after including the quantifier.
%     This last step generates rule 3, which matches all sententences.
%     The three sentences compose the specification along with the final rule.
%   }
% \label{data-generation-example}
% \end{figure}
% \label{sss:training_data}

